One-Step Diffusion for Detail-Rich and Temporally Consistent Video Super-Resolution

It is a challenging problem to reproduce rich spatial details while maintaining temporal consistency in real-world video super-resolution (Real-VSR), especially when we leverage pre-trained generative models such as stable diffusion (SD) for realistic details synthesis. Existing SD-based Real-VSR methods often compromise spatial details for temporal coherence, resulting in suboptimal visual quality. We argue that the key lies in how to effectively extract the degradation-robust temporal consistency priors from the low-quality (LQ) input video and enhance the video details while maintaining the extracted consistency priors. To achieve this, we propose a Dual LoRA Learning (DLoRAL) paradigm to train an effective SD-based one-step diffusion model, achieving realistic frame details and temporal consistency simultaneously. Specifically, we introduce a Cross-Frame Retrieval (CFR) module to aggregate complementary information across frames, and train a Consistency-LoRA (C-LoRA) to learn robust temporal representations from degraded inputs. After consistency learning, we fix the CFR and C-LoRA modules and train a Detail-LoRA (D-LoRA) to enhance spatial details while aligning with the temporal space defined by C-LoRA to keep temporal coherence. The two phases alternate iteratively for optimization, collaboratively delivering consistent and detail-rich outputs. During inference, the two LoRA branches are merged into the SD model, allowing efficient and high-quality video restoration in a single diffusion step. Experiments show that DLoRAL achieves strong performance in both accuracy and speed. Code and models are available at https://github.com/yjsunnn/DLoRAL.

==> chapters/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the main claims in the abstract and introduction accurately reflect the paper's contributions and scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss limitations in the final section (after the conclusion).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper provides a full set of assumptions and a proof for each theoretical result.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper fully discloses all necessary information to reproduce the main experimental results, supporting the main claims and conclusions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All data are publicly available. We will release the codes and new data if the paper is accepted.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the paper provides all necessary details, including hyperparameters, evaluation metrics and \textit{etc.} to fully understand the results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not report error bars.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail the type of compute resources in experimental settings.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the research in the paper fully conforms to the NeurIPS Code of Ethics in every respect.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we analyze the potential social impact in appendix.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, we clearly indicate the baseline methods and testing data used in the paper. Their licenses permit use with academic scope.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code and dataset will be release if the paper is accepted.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowd sourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowd sourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our core method focuses on video super-resolution and does not involve LLMs as part. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> chapters/experiment.tex <==
\section{Experiment}
\label{exp}
\subsection{Experimental Settings}
\noindent\textbf{Implementation Details.} %The training of our Dual-LoRA framework consists of two iterative stages: consistency modeling and detail enhancement. 
We adopt the pre-trained Stable Diffusion V2.1 as the backbone of denoising U-Net. Training is carried out with a batch size of 16, a sequence length of 3, and a video resolution of $512 \times 512$.
All models are trained using the PyTorch framework on 4 NVIDIA A100 GPUs. We use Adam optimizer with an initial learning rate of $5\times10^{-5}$. For inference, both C-LoRA and D-LoRA are activated simultaneously in a frozen UNet. Videos are processed in sliding sequences to fit GPU memory limits. %A single forward pass generates each output frame to ensure real-time performance.

% training datasets: 对于consistency stage阶段，数据需要保证其运动的真实性、时序的连续性，在此基础上需要保证一定的高质量；因此我们从(1)REDS dataset (2)Pexel video这两个video dataset中筛选出了相对高质量的44k图像用来做consistency stage的训练；对于enhancement stage阶段，数据需要高质量、涵盖丰富场景，同时帧间要有一定的运动，防止模型遗忘上一阶段学到的内容。因此我们从（3）LSDIR数据集中合成了video数据集，采用shift整数个pixel位置的方式stimulate运动同时又不影响画质，得到的高质量stimulated video数据集用来训练enhancement stage。这两个阶段中的所有数据，都采用RealESRGAN的方式进行退化，同一个视频中的不同帧采用相同的退化参数以模拟现实场景中的拍摄条件，不同的视频则采用随机的退化参数。
% testing datasets: 
\noindent\textbf{Training Datasets.} To support the decoupled training design of our DLoRAL framework, we construct two training datasets for the consistency and enhancement stages, respectively.

For the \textit{\textbf{consistency stage}}, the training data needs to contain realistic motion while maintaining reasonable image quality. To this end, we select 44,162 high-quality frames from the REDS dataset~\cite{nah2019REDS}, which offers professionally captured sequences with rich dynamics, and a curated set of videos~\cite{wu2025insvie} from Pexels\footnote{\url{https://www.pexels.com/}}, chosen based on aesthetic and temporal smoothness criteria. These sequences provide necessary temporal priors for learning degradation-robust representations.

For the \textit{\textbf{enhancement stage}}, the training data should prioritize visual quality. Thus, we select the LSDIR~\cite{li2023lsdir} dataset, known for its rich textures and fine-grained details. To preserve the learned consistency modeling capability and enable the optical flow regularization among frames, we generate simulated video sequences based on LSDIR. Specifically, for each ground-truth image in LSDIR, we apply random pixel-level translations to it to generate multiple shifted images.

The data in both stages are degraded using the RealESRGAN~\cite{wang2021realesrgan} degradation pipeline. %, which involves combinations of blur, noise, downsampling, and compression. To simulate realistic capture conditions, 
We apply identical degradation parameters across frames within the same video, while using random parameters for different video sequences.

\textbf{Testing Datasets.} We evaluate our method on both synthetic and real-world datasets, including UDM10~\cite{yi2019UDM10}, SPMCS~\cite{tao2017SPMCS}, RealVSR~\cite{yang2021realvsr}, and VideoLQ~\cite{chan2022realbasicvsr}. Among them, UDM10 contains 10 sequences, each having 32 frames. SPMCS contains 30 sequences, each having 31 frames. RealVSR contains 50 real-world sequences, each having 50 frames. VideoLQ contains 50 real-world sequences with complex degradations. For the synthetic dataset (UDM10 and SPMCS), we synthesize LQ-HQ pairs following the same degradation pipeline in training. For real-world datasets (RealVSR and VideoLQ), we directly adopt the given LQ-HQ pairs.

\noindent\textbf{Evaluation Metrics.}
A set of full-reference and no-reference metrics are selected to evaluate different real-world VSR methods. The full-reference metrics include PSNR and SSIM, and perceptual quality with LPIPS~\cite{zhang2018lpips} and DISTS~\cite{ding2020dists}.
No-reference quality assessment involves MUSIQ~\cite{ke2021musiq}, MANIQA~\cite{yang2022maniqa}, CLIPIQA~\cite{wang2023clipiqa}, and the video quality assessment metric DOVER~\cite{wu2023dover}.
Compared to Real-ISR, Real-VSR places greater emphasis on temporal consistency. Following prior works~\cite{yang2024motion, zhang2024tmp}, we use the average warping error $E^*_{warp}$ to quantitatively assess temporal consistency: $E^*_{warp} = \frac{1}{N-1} \sum_{i=1}^{N-1} || I_{i+1}^{HQ} - F_{wp}(I_i^{HQ}) ||_1$. 
For the test datasets with GT, optical flow in $F_{wp}$ is estimated from GT frames. For real-world datasets without GT (\textit{e.g.}, VideoLQ test set), we use the flow estimated from predicted frames.


\subsection{Experimental Results}
To demonstrate the effectiveness of our DLoRAL algorithm, we compare it with seven represnetative and state-of-the-art methods, including three Real-ISR models (RealESRGAN~\cite{wang2021realesrgan}, StableSR~\cite{wang2024stablesr}, and the one-step model OSEDiff~\cite{wu2024osediff}), a discriminative VSR model (RealBasicVSR~\cite{chan2022realbasicvsr}), and three diffusion-based VSR models (Upscale-A-Video~\cite{zhou2024upscale}, MGLD-VSR~\cite{yang2024motion} and STAR~\cite{xie2025star}).



% \begin{table}
% \centering
% \setlength{\tabcolsep}{3pt} % 调整列间距
% \renewcommand{\arraystretch}{1.2} % 调整行间距
% \resizebox{\textwidth}{!}{ % 自动缩放表格宽度
% \begin{tabular}{|c|c||c|c|c||c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Datasets} & \multirow{2}{*}{Metrics} & \multicolumn{3}{c||}{Real-ISR Methods} & \multicolumn{5}{c|}{Real-VSR Methods} \\
% \cline{3-10}
% & & RealESRGSN & StableSR  &OSEDiff 
% & RealBasicVSR & Upscale-A-Video & MGLD & STAR & \textbf{DLoRAL} \\ \hline
% \multirow{10}{*}{UDM10}
%  & PSNR $\uparrow$ & 21.34 & 22.04  &23.76 
% & \textcolor{blue}{\textbf{24.33}} & 22.36 & 24.19 & \textcolor{red}{\textbf{24.45}} & 23.97 \\ 
%  & SSIM $\uparrow$ & 0.5650 & 0.5680  &0.6964 
% & \textcolor{red}{\textbf{0.7225}} & 0.5836 & 0.6845 & \textcolor{blue}{\textbf{0.7143}} & 0.7104 \\ 
%  & LPIPS $\downarrow$ & 0.4510 & 0.4550  &0.3666 
% & 0.3629 & 0.4097 & \textcolor{blue}{\textbf{0.3354}} & 0.4165 & \textcolor{red}{\textbf{0.3269}} \\
%  & DISTS $\downarrow$ &  \textcolor{red}{\textbf{0.1750}} & 0.1850  & \textcolor{blue}{\textbf{0.1754}} 
% & 0.2042 & 0.1980 & 0.1763 & 0.2299 & 0.1786 \\ 
%  & BRISQUE $\downarrow$ & 29.8433 & 26.3090  &20.7179 
% & \textcolor{red}{\textbf{14.1290}} & 17.6070 & 22.7012 & 36.9100 & \textcolor{blue}{\textbf{16.2501}} \\ 
%  & MUSIQ $\uparrow$ & 49.8380 & 47.8050  & \textcolor{blue}{\textbf{63.1462}} 
% & 62.3600 & 61.0457 & 61.3086 & 40.789 & \textcolor{red}{\textbf{65.6201}} \\
%  & CLIPIQA $\uparrow$ & 0.4740 & 0.4452  &\textcolor{blue}{\textbf{0.5741}} 
% & 0.4741 & 0.4448 & 0.4534 & 0.2671 & \textcolor{red}{\textbf{0.6518}} \\
%  & MANIQA $\uparrow$ & 0.3302 & 0.3185  &\textcolor{blue}{\textbf{0.3342}} 
% & 0.3295 & 0.3184 & 0.2906 & 0.2443 & \textcolor{red}{\textbf{0.3727}} \\
%  & \(E^{*}_\text{warp}\) $\downarrow$ & 7.58 & 8.44  &5.22 
% & 4.67 & 5.79 & \textcolor{blue}{\textbf{4.61}} & \textcolor{red}{\textbf{3.51}} & 4.72 \\
%  & DOVER $\uparrow$ & 36.8600 & 30.4702  &\textcolor{red}{\textbf{48.4044}} 
% & 37.5723 & 37.6941 & 40.0445 & 30.3836 &  \textcolor{blue}{\textbf{42.8714}}\\ \hline
% \multirow{10}{*}{SPMCS} 
%  & PSNR $\uparrow$ & \textcolor{red}{\textbf{21.66}} & 19.26  &20.65 
% & \textcolor{blue}{\textbf{21.58}} & 19.03 & 21.26 & 20.73 & 21.24 \\ 
%  & SSIM $\uparrow$ & 0.5691 & \textcolor{blue}{\textbf{0.5847}}  &\textcolor{red}{\textbf{0.6963}} 
% & 0.5447 & 0.3860 & 0.5148 & 0.4888 & 0.5239 \\ 
%  & LPIPS $\downarrow$ & 0.4441 & 0.4323  &\textcolor{red}{\textbf{0.3537}} 
% & 0.4038 & 0.4850 & 0.3838 & 0.6064 & \textcolor{blue}{\textbf{0.3754}} \\ 
%  & DISTS $\downarrow$ & 0.2455 & 0.2354  & \textcolor{blue}{\textbf{0.2291}} 
% & 0.2368 & 0.2741 & 0.2339 & 0.3418 & \textcolor{red}{\textbf{0.2216}} \\ 
%  & BRISQUE $\downarrow$ & 25.2404 & 26.3095  &19.4713 
% & 12.0483 & \textcolor{blue}{\textbf{19.7841}} & 23.1835 & 27.9015 & \textcolor{red}{\textbf{11.0296}} \\ 
%  & MUSIQ $\uparrow$ & 53.2210 & 47.8050  &64.6191 
% & 66.6827 &\textcolor{blue}{\textbf{66.9116}} & 65.0792 & 33.2473 & \textcolor{red}{\textbf{67.3900}} \\
%  & CLIPIQA $\uparrow$ & 0.5151 & 0.4450  &\textcolor{blue}{\textbf{0.5259}} 
% & 0.5149 & 0.5170 & 0.4371 & 0.2403 & \textcolor{red}{\textbf{0.5805}} \\
%  & MANIQA $\uparrow$ & 0.3081 & 0.3186  &0.3081 
% & 0.3079 & \textcolor{red}{\textbf{0.4425}} & 0.3123 & 0.2370 & \textcolor{blue}{\textbf{0.3402}} \\
%  & \(E^{*}_\text{warp}\) $\downarrow$ & 7.57 & 8.43  &7.50
% & 5.40 & 7.57 & \textcolor{blue}{\textbf{4.41}} & \textcolor{red}{\textbf{4.08}} & 6.25 \\
%  & DOVER $\uparrow$ & 32.151 & 30.470  &\textcolor{red}{\textbf{40.160}} 
% & 30.953 & 32.151 & 31.1177 & 17.22 & \textcolor{blue}{\textbf{34.895}} \\ \hline
% \multirow{10}{*}{RealVSR} 
%  & PSNR $\uparrow$ & \textcolor{blue}{\textbf{21.34}} & 18.95  &19.92
% & \textcolor{red}{\textbf{22.27}} & 20.06 & 21.12 & 15.08 & 20.36 \\ 
%  & SSIM $\uparrow$ & 0.5651 & 0.5830  &0.5878 
% &\textcolor{red}{\textbf{0.7195}} & 0.5908 &\textcolor{blue}{\textbf{0.6460}} & 0.4328 &  0.6063 \\ 
%  & LPIPS $\downarrow$ & 0.4510 & 0.2254  &0.2820 
% & \textcolor{red}{\textbf{0.1929}} & 0.2631 & \textcolor{blue}{\textbf{0.2194}} & 0.4085 & 0.2422 \\
%  & DISTS $\downarrow$ & 0.175 & 0.154  &0.1638 
% & 0.1598 & 0.1584 & \textcolor{blue}{\textbf{0.1512}} & 0.2785 & \textcolor{red}{\textbf{0.1497}} \\ 
%  & BRISQUE $\downarrow$ & 29.8435 & 28.2504  &31.7940 
% & 30.3622 & \textcolor{red}{\textbf{25.4762}} & 39.0817 & 62.7500 & \textcolor{blue}{\textbf{27.8931}} \\ 
%  & MUSIQ $\uparrow$ & 49.8381 & 69.9615  &64.1013 
% & \textcolor{red}{\textbf{71.4127}} & 67.7141 & 70.7340 & 67.9470 & \textcolor{blue}{\textbf{70.9081}}\\ 
%  & CLIPIQA $\uparrow$ & 0.4744 & \textcolor{blue}{\textbf{0.6124}}  &0.5455 
% & 0.3699 & 0.4355 & 0.5295 & 0.5318 & \textcolor{red}{\textbf{0.6165}} \\ 
%  & MANIQA $\uparrow$ & 0.3301 & 0.3452  &0.3407 
% & 0.3836 & \textcolor{blue}{\textbf{0.4139}} & \textcolor{red}{\textbf{0.4960}} & 0.4383 & 0.3861 \\ 
%   & \( E^{*}_\text{warp}\) $\downarrow$ & 17.5800 & 25.01  &18.3 
% & 18.72 & \textcolor{blue}{\textbf{18.20}} & 19.21 & 24.6 & \textcolor{red}{\textbf{17.30}} \\
%  & DOVER $\uparrow$ & 36.8600 & \textcolor{blue}{\textbf{46.8461}}  &42.1382 
% & 46.4388 & 36.1364 & 42.0438 & 30.2139 & \textcolor{red}{\textbf{49.6456}} \\ \hline
% \multirow{6}{*}{VideoLQ} 
%  & BRISQUE $\downarrow$ & 29.6050 & \textcolor{red}{\textbf{22.3370}}  &26.4025 
% & 24.7904 & 25.1011 & 29.6062 & 42.5818 & \textcolor{blue}{\textbf{23.0393}} \\ 
%  & MUSIQ $\uparrow$ & 53.138 & 52.975  &58.9585 
% & \textcolor{blue}{\textbf{59.4750}} & 57.4886 & 53.0915 & 49.3046 & \textcolor{red}{\textbf{63.8463}}\\
%  & CLIPIQA $\uparrow$ & 0.334 & 0.478  & \textcolor{blue}{\textbf{0.499}} 
% & 0.3930 & 0.3772 & 0.3145 & 0.3328 & \textcolor{red}{\textbf{0.567}}\\
%  & MANIQA $\uparrow$ & 0.232 & 0.278  &0.2542 
% & 0.3115 & \textcolor{blue}{\textbf{0.3275}} & 0.2542 & 0.2682 & \textcolor{red}{\textbf{0.3442}}\\
%  & \(E^*_\text{warp}\) $\downarrow$ & 7.58 & 8.43  &8.406 
% & 8.1075 & 7.586 & \textcolor{blue}{\textbf{7.409}} & \textcolor{red}{\textbf{7.28}} & 7.897 \\
%  & DOVER $\uparrow$ & 28.40 & 30.47  & \textcolor{blue}{\textbf{37.58}} & 34.7721 & 36.86 & 31.8992 & 29.40 & \textcolor{red}{\textbf{38.5054}} \\ \hline
% \end{tabular}
% }
% \vspace{10pt}
% \caption{Comparison of various Real-ISR and Real-VSR methods across different datasets. The best and second
% best results of each metric are highlighted in \textcolor{red}{\textbf{red}} and \textcolor{blue}{\textbf{blue}}, respectively.}
% \label{tab:comparison}
% \end{table}

\begin{table}
\centering
\setlength{\tabcolsep}{3pt} % 调整列间距
\renewcommand{\arraystretch}{1.2} % 调整行间距
\resizebox{\textwidth}{!}{ % 自动缩放表格宽度
\begin{tabular}{|c|c||c|c|c||c|c|c|c|c|}
\hline
\multirow{2}{*}{Datasets} & \multirow{2}{*}{Metrics} & \multicolumn{3}{c||}{Real-ISR Methods} & \multicolumn{5}{c|}{Real-VSR Methods} \\
\cline{3-10}
& & RealESRGSN & StableSR  & OSEDiff 
& RealBasicVSR & Upscale-A-Video & MGLD & STAR & \textbf{DLoRAL} \\ \hline
\multirow{10}{*}{UDM10}
 & PSNR $\uparrow$ & 21.345 & 22.042 & 23.761 
& \textcolor{blue}{\textbf{24.334}} & 22.364 & 24.192 & \textcolor{red}{\textbf{24.451}} & 23.975 \\ 
 & SSIM $\uparrow$ & 0.565 & 0.568 & 0.696 
& \textcolor{red}{\textbf{0.723}} & 0.584 & 0.685 & \textcolor{blue}{\textbf{0.714}} & 0.710 \\ 
 & LPIPS $\downarrow$ & 0.451 & 0.455 & 0.367 
& 0.363 & 0.410 & \textcolor{blue}{\textbf{0.335}} & 0.417 & \textcolor{red}{\textbf{0.327}} \\
 & DISTS $\downarrow$ & \textcolor{red}{\textbf{0.175}} & 0.185 & \textcolor{blue}{\textbf{0.175}} 
& 0.204 & 0.198 & 0.176 & 0.230 & 0.179 \\ 
 & BRISQUE $\downarrow$ & 29.843 & 26.310 & 20.718 
& \textcolor{red}{\textbf{14.129}} & 17.607 & 22.701 & 36.910 & \textcolor{blue}{\textbf{16.250}} \\ 
 & MUSIQ $\uparrow$ & 49.838 & 47.805 & \textcolor{blue}{\textbf{63.146}} 
& 62.360 & 61.046 & 61.309 & 40.789 & \textcolor{red}{\textbf{65.620}} \\
 & CLIPIQA $\uparrow$ & 0.474 & 0.445 & \textcolor{blue}{\textbf{0.574}} 
& 0.474 & 0.445 & 0.453 & 0.267 & \textcolor{red}{\textbf{0.652}} \\
 & MANIQA $\uparrow$ & 0.330 & 0.319 & \textcolor{blue}{\textbf{0.334}} 
& 0.330 & 0.318 & 0.291 & 0.244 & \textcolor{red}{\textbf{0.373}} \\
 & \(E^{*}_\text{warp}\) $\downarrow$ & 7.580 & 8.440 & 5.220 
& 4.670 & 5.790 & \textcolor{blue}{\textbf{4.610}} & \textcolor{red}{\textbf{3.510}} & 4.720 \\
 & DOVER $\uparrow$ & 36.860 & 30.470 & \textcolor{red}{\textbf{48.404}} 
& 37.572 & 37.694 & 40.045 & 30.384 & \textcolor{blue}{\textbf{42.871}} \\ \hline
\multirow{10}{*}{SPMCS} 
 & PSNR $\uparrow$ & \textcolor{red}{\textbf{21.660}} & 19.260 & 20.650 
& \textcolor{blue}{\textbf{21.580}} & 19.030 & 21.260 & 20.730 & 21.240 \\ 
 & SSIM $\uparrow$ & 0.569 & \textcolor{blue}{\textbf{0.585}} & \textcolor{red}{\textbf{0.696}} 
& 0.545 & 0.386 & 0.515 & 0.489 & 0.524 \\ 
 & LPIPS $\downarrow$ & 0.444 & 0.432 & \textcolor{red}{\textbf{0.354}} 
& 0.404 & 0.485 & 0.384 & 0.606 & \textcolor{blue}{\textbf{0.375}} \\ 
 & DISTS $\downarrow$ & 0.246 & 0.235 & \textcolor{blue}{\textbf{0.229}} 
& 0.237 & 0.274 & 0.234 & 0.342 & \textcolor{red}{\textbf{0.222}} \\ 
 & BRISQUE $\downarrow$ & 25.240 & 26.310 & 19.471 
& 12.048 & \textcolor{blue}{\textbf{19.784}} & 23.184 & 27.902 & \textcolor{red}{\textbf{11.030}} \\ 
 & MUSIQ $\uparrow$ & 53.221 & 47.805 & 64.619 
& 66.683 & \textcolor{blue}{\textbf{66.912}} & 65.079 & 33.247 & \textcolor{red}{\textbf{67.390}} \\
 & CLIPIQA $\uparrow$ & 0.515 & 0.445 & \textcolor{blue}{\textbf{0.526}} 
& 0.515 & 0.517 & 0.437 & 0.240 & \textcolor{red}{\textbf{0.581}} \\
 & MANIQA $\uparrow$ & 0.308 & 0.319 & 0.308 
& 0.308 & \textcolor{red}{\textbf{0.443}} & 0.312 & 0.237 & \textcolor{blue}{\textbf{0.340}} \\
 & \(E^{*}_\text{warp}\) $\downarrow$ & 7.570 & 8.430 & 7.500 
& 5.400 & 7.570 & \textcolor{blue}{\textbf{4.410}} & \textcolor{red}{\textbf{4.080}} & 6.250 \\
 & DOVER $\uparrow$ & 32.151 & 30.470 & \textcolor{red}{\textbf{40.160}} 
& 30.953 & 32.151 & 31.118 & 17.220 & \textcolor{blue}{\textbf{34.895}} \\ \hline
\multirow{10}{*}{RealVSR} 
 & PSNR $\uparrow$ & \textcolor{blue}{\textbf{21.340}} & 18.950 & 19.920 
& \textcolor{red}{\textbf{22.270}} & 20.060 & 21.120 & 15.080 & 20.360 \\ 
 & SSIM $\uparrow$ & 0.565 & 0.583 & 0.588 
& \textcolor{red}{\textbf{0.720}} & 0.591 & \textcolor{blue}{\textbf{0.646}} & 0.433 & 0.606 \\ 
 & LPIPS $\downarrow$ & 0.451 & 0.225 & 0.282 
& \textcolor{red}{\textbf{0.193}} & 0.263 & \textcolor{blue}{\textbf{0.219}} & 0.409 & 0.242 \\
 & DISTS $\downarrow$ & 0.175 & 0.154 & 0.164 
& 0.160 & 0.158 & \textcolor{blue}{\textbf{0.151}} & 0.279 & \textcolor{red}{\textbf{0.150}} \\ 
 & BRISQUE $\downarrow$ & 29.843 & 28.250 & 31.794 
& 30.362 & \textcolor{red}{\textbf{25.476}} & 39.082 & 62.750 & \textcolor{blue}{\textbf{27.893}} \\ 
 & MUSIQ $\uparrow$ & 49.838 & 69.962 & 64.101 
& \textcolor{red}{\textbf{71.413}} & 67.714 & 70.734 & 67.947 & \textcolor{blue}{\textbf{70.908}} \\
 & CLIPIQA $\uparrow$ & 0.474 & \textcolor{blue}{\textbf{0.612}} & 0.546 
& 0.370 & 0.436 & 0.530 & 0.532 & \textcolor{red}{\textbf{0.617}} \\ 
 & MANIQA $\uparrow$ & 0.330 & 0.345 & 0.341 
& 0.384 & \textcolor{blue}{\textbf{0.414}} & \textcolor{red}{\textbf{0.496}} & 0.438 & 0.386 \\ 
  & \(E^{*}_\text{warp}\) $\downarrow$ & 17.580 & 25.010 & 18.300 
& 18.720 & \textcolor{blue}{\textbf{18.200}} & 19.210 & 24.600 & \textcolor{red}{\textbf{17.300}} \\
 & DOVER $\uparrow$ & 36.860 & \textcolor{blue}{\textbf{46.846}} & 42.138 
& 46.439 & 36.136 & 42.044 & 30.214 & \textcolor{red}{\textbf{49.646}} \\ \hline
\multirow{6}{*}{VideoLQ} 
 & BRISQUE $\downarrow$ & 29.605 & \textcolor{red}{\textbf{22.337}} & 26.403 
& 24.790 & 25.101 & 29.606 & 42.582 & \textcolor{blue}{\textbf{23.039}} \\ 
 & MUSIQ $\uparrow$ & 53.138 & 52.975 & 58.959 
& \textcolor{blue}{\textbf{59.475}} & 57.489 & 53.092 & 49.305 & \textcolor{red}{\textbf{63.846}} \\
 & CLIPIQA $\uparrow$ & 0.334 & 0.478 & \textcolor{blue}{\textbf{0.499}} 
& 0.393 & 0.377 & 0.315 & 0.333 & \textcolor{red}{\textbf{0.567}} \\
 & MANIQA $\uparrow$ & 0.232 & 0.278 & 0.254 
& 0.312 & \textcolor{blue}{\textbf{0.328}} & 0.254 & 0.268 & \textcolor{red}{\textbf{0.344}} \\
 & \(E^*_\text{warp}\) $\downarrow$ & 7.580 & 8.430 & 8.406 
& 8.108 & 7.586 & \textcolor{blue}{\textbf{7.409}} & \textcolor{red}{\textbf{7.280}} & 7.897 \\
 & DOVER $\uparrow$ & 28.400 & 30.470 & \textcolor{blue}{\textbf{37.580}} 
& 34.772 & 36.860 & 31.899 & 29.400 & \textcolor{red}{\textbf{38.505}} \\ \hline
\end{tabular}
}
\vspace{5pt}
\caption{Comparison of various Real-ISR and Real-VSR methods across different datasets. The best and second
best results of each metric are highlighted in \textcolor{red}{\textbf{red}} and \textcolor{blue}{\textbf{blue}}, respectively.}
\label{tab:comparison}
\vspace{-25pt}
\end{table}


\noindent\textbf{Quantitative Comparison.}
We show the quantitative comparison on both synthetic and real-world video benchmarks in Tab~\ref{tab:comparison}, from which several key observations can be made.
First, non-diffusion-based methods (\textit{e.g.}, RealESRGAN and RealBasicVSR) perform worse than diffusion-based methods on no-reference perceptual quality metrics, such as MUSIQ and CLIPIQA, mainly because they lack the strong image priors provided by pre-trained SD models, leading to over-smoothed results. 
Second, SD-based Real-ISR methods (StableSR and OSEDiff) can achieve comparable or even better perceptual quality scores than existing Real-VSR methods. In particular, OSEDiff achieves the best DOVER scores on both the UDM10 and SPMCS datasets. However, its warping error evaluated by $E^*_{warp}$ is worse. This is because the Real-ISR methods generate details for each frame without considering the inter-frame consistency.
% \textcolor{blue}{This is because, two synthetic datasets are synthesized using extremely severe degradation parameters, where details are invisible in the inputs. Visual quality oriented methods could handle these cases by generating the optimal visual-quality for each frame, which is favored by measurement of DOVER. However, the corresponding consequence is the high warping error on $E^*_{warp}$. As the generated details change from frames to frames, leading to flickering effects.}
Finally, compared to the existing Real-VSR methods, our DLoRAL consistently ranks first or second across a range of perceptual quality metrics, including LPIPS, DISTS, MUSIQ, CLIPIQA, MANIQA, and DOVER, demonstrating its strong alignment with human perception. 
At the same time, DLoRAL does not compromise temporal consistency, as evidenced by its superior performance on the $E^*_{warp}$ metric. For example, on the RealVSR dataset, DLoRAL achieves state-of-the-art results in DISTS, CLIPIQA, and DOVER, while ranking among the top in $E^*_{warp}$, highlighting its ability to produce visually pleasing and temporally coherent outputs.

It should be mentioned that although $E^*_{warp}$ is widely used to assess temporal consistency, it does not correlate well with human perception. For example, blurry Real-VSR outputs can achieve lower warping errors but exhibit poorer visual quality.
DLoRAL may report slightly larger $E^*_{warp}$ values than some methods (\textit{e.g.}, STAR), but this is because DLoRAL better preserves fine details that the warping error metric tends to penalize.

% While the warping error (WE) metric is widely adopted for temporal consistency evaluation, it should be noted that this measurement does not always correlate with human perception of video quality. The metric can be artificially inflated by simply blurring the output sequence—a manipulation that improves WE scores while actually degrading visual quality. As evidenced in Table~\ref{tab:comparison}, our method achieves relatively higher WE values compared to some VSR approaches, which primarily stems from its superior ability to reconstruct fine details and textures that the WE metric inherently penalizes.



% We show the quantitative comparison on both synthetic and real-world video benchmarks in Tab~\ref{tab:comparison}. The table highlights several key observations.
% First, non-diffusion-based methods (\textit{e.g.}, RealESRGAN and RealBasicVSR) perform worse than diffusion-based methods on no-reference perceptual quality metrics, such as MUSIQ and CLIPIQA. This is because they lack the natural image priors provided by pre-trained diffusion models, often leading to over-smoothed results. 
% Second, Real-ISR methods can achieve comparable or even better quality scores than Real-VSR methods. For example, OSEDiff achieves the best DOVER scores on both the UDM10 and SPMCS datasets.
% However, Real-ISR methods typically perform worse in temporal consistency on $E^*_{warp}$, as they are not designed to model inter-frame coherence.
% Finally, compared to other Real-VSR methods, the proposed DLoRAL consistently achieves top or second-best performance on perceptual quality metrics such as LPIPS, DISTS, MUSIQ, CLIPIQA, MANIQA, and DOVER, demonstrating its ability to generate visually pleasing results aligned with human perception. Notably, on the UDM10 dataset, DLoRAL outperforms MGLD in MUSIQ by over 4 points (65.62 vs. 61.31), and even surpasses the best Real-ISR method, OSEDiff (63.15).
% Moreover, DLoRAL achieves competitive temporal consistency, with the best $E^*_{warp}$ score on the RealVSR dataset, showing that it can produce both high-quality and temporally stable video frames. More discussion of $E^*_{warp}$ can be found in the following.



% We first show the quantitative comparison on both synthetic and real-world video benchmarks in Tab~\ref{tab:comparison}. As shown from Tab~\ref{tab:comparison}, our method achieves outperforming results across all datasets in terms of perceptual quality metrics including MUSIQ, CLIPIQA, MANIQA and DOVER, demonstrating superior capability in generating visually pleasing results that align well with human perception. The proposed method also obtains the top performance in DISTS scores on two (SPMCS and RealVSR) out of three test datasets with references, indicating its strong ability to reconstruct high-quality plausible details under various degradation conditions. While some methods like RealBasicVSR achieve better performance in traditional fidelity metrics such as PSNR or SSIM on certain datasets, our approach consistently delivers more visually appealing results, as evidenced by the perceptual metrics. For the Real-VSR task, our method establishes new state-of-the-art performance on the VideoLQ benchmark, achieving the best results in all no-reference quality metrics, including BRISQUE, MUSIQ, CLIPIQA, and MANIQA. The superior and consistent performance across both synthetic and real-world datasets verifies the effectiveness of our method in handling various real-world degradations while maintaining temporal coherence and producing realistic details.



% \begin{table}[htbp]
% \centering
% \setlength{\tabcolsep}{3pt} % 调整列间距
% \renewcommand{\arraystretch}{1.2} % 调整行间距
% \resizebox{\textwidth}{!}{ % 自动缩放表格宽度
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Datasets} & \textbf{Metrics} & \textbf{RealESRGSN} & \textbf{OSEDiff} & \textbf{StableSR} & \textbf{RealBasicVSR} & \textbf{Upscale-A-Video} & \textbf{MGLD} & \textbf{STAR} & \textbf{Ours} \\ \hline
% % \multirow{9}{*}{UDM10} 
% \multirow{10}{*}{UDM10}
%  & PSNR $\uparrow$ & -- & 23.764 & -- & 24.3317 & 22.357 & 24.1901 & 24.4492 & 23.968 \\ 
%  & SSIM $\uparrow$ & -- & 0.69637 & -- & 0.7225 & 0.5836 & 0.6845 & 0.7143 & 0.7104 \\ 
%  & LPIPS $\downarrow$ & -- & 0.3666 & -- & 0.3629 & 0.4097 & 0.3354 & 0.4165 & \textcolor{red}{0.3269} \\
%  & DISTS $\downarrow$ & -- & 0.1754 & -- & 0.2042 & 0.1980 & 0.1763 & 0.2299 & 0.1786 \\ 
%  & BRISQUE $\downarrow$ & -- & 20.7179 & -- & \textcolor{red}{14.129} & 17.607 & 22.701 & 36.9100 & \textcolor{blue}{16.250} \\ 
%  & MUSIQ $\uparrow$ & -- & 63.1462 & -- & 62.3600 & 61.0457 & 61.3086 & 40.789 & \textcolor{red}{65.6201} \\
%  & CLIPIQA $\uparrow$ & -- & 0.5741 & -- & 0.4741 & 0.4448 & 0.4534 & 0.2671 & \textcolor{red}{0.6518} \\
%  & MANIQA $\uparrow$ & -- & 0.3342 & -- & 0.3295 & 0.3184 & 0.2906 & 0.244 & \textcolor{red}{0.372} \\
%  & \(E^{*}_\text{warp}\) $\downarrow$ & -- & 5.22 & -- & 4.673 & 5.79 & 4.61 & 3.51 & 4.7232 \\
%  & DOVER $\uparrow$ & -- & \textcolor{red}{48.4044} & -- & 37.572 & 37.694 & 40.0445 & 30.383 &  \textcolor{blue}{42.8714}\\ \hline
% \multirow{10}{*}{SPMCS} 
%  & PSNR $\uparrow$ & -- & 20.6524 & -- & 21.582 & 19.034 & 21.258 & 20.727 & 21.2363 \\ 
%  & SSIM $\uparrow$ & -- & 0.6963 & -- & 0.5447 & 0.386 & 0.5148 & 0.4888 & 0.5239 \\ 
%  & LPIPS $\downarrow$ & -- & \textcolor{red}{0.35373} & -- & 0.4038 & 0.485 & 0.3838 & 0.6064 & \textcolor{blue}{0.3754} \\ 
%  & DISTS $\downarrow$ & -- & 0.229 & -- & 0.2368 & 0.274 & 0.233 & 0.3418 & \textcolor{red}{0.2216} \\ 
%  & BRISQUE $\downarrow$ & -- & 19.4713 & -- & 12.0483 & 19.784 & 23.1835 & 27.9015 & \textcolor{red}{11.0296} \\ 
%  & MUSIQ $\uparrow$ & -- & 64.619 & -- & 66.6827 & 66.911 & 65.0792 & 33.247 & \textcolor{red}{67.390} \\
%  & CLIPIQA $\uparrow$ & -- & 0.5259 & -- & 0.5149 & 0.517 & 0.4371 & 0.2403 & \textcolor{red}{0.58048} \\
%  & MANIQA $\uparrow$ & -- & 0.3081 & -- & 0.3079 & \textcolor{red}{0.4425} & 0.3123 & 0.2370 & \textcolor{blue}{0.3402} \\
%  & \(E^{*}_\text{warp}\) $\downarrow$ & -- & 7.495 & -- & 5.399 & 7.573 & 4.411 & 4.075 & 6.2489 \\
%  & DOVER $\uparrow$ & -- & \textcolor{red}{40.160} & -- & 30.953 & 32.151 & 31.1177 & 17.22 & \textcolor{blue}{34.895} \\ \hline
% \multirow{10}{*}{RealVSR} 
%  & PSNR $\uparrow$ & -- & 19.917 & 18.948 & 22.2708 & 20.060 & 21.1163 & 15.078 & 20.3639 \\ 
%  & SSIM $\uparrow$ & -- & 0.5878 & 0.583 & 0.7195 & 0.5908 & 0.6460 & 0.432 &  0.6063 \\ 
%  & LPIPS $\downarrow$ & -- & 0.2820 & 0.225 & \textcolor{red}{0.1929} & 0.2631 & 0.2194 & 0.4085 & 0.2422 \\
%  & DISTS $\downarrow$ & -- & 0.1638 & 0.154 & 0.1598 & 0.1584 & \textcolor{blue}{0.1512} & 0.2785 & \textcolor{red}{0.1497} \\ 
%  & BRISQUE $\downarrow$ & -- & 31.794 & 28.250 & 30.3622 & \textcolor{red}{25.476} & 39.081 & 62.750 & \textcolor{blue}{27.893} \\ 
%  & MUSIQ $\uparrow$ & -- & 64.101 & 69.961 & \textcolor{red}{71.412} & 67.714 & 70.734 & 67.947 & \textcolor{blue}{70.908}\\ 
%  & CLIPIQA $\uparrow$ & -- & 0.5455 & 0.6124 & 0.3699 & 0.435 & 0.5295 & 0.5318 & \textcolor{red}{0.61654} \\ 
%  & MANIQA $\uparrow$ & -- & 0.34069 & -- & 0.3836 & \textcolor{blue}{0.4139} & \textcolor{red}{0.4960} & 0.4383 & 0.3861 \\ 
%   & \( E^{*}_\text{warp}\) $\downarrow$ & -- & 18.3 & 25.01 & 18.72 & \textcolor{blue}{18.2} & 19.2 & 34.6 & \textcolor{red}{17.3} \\
%  & DOVER $\uparrow$ & -- & 42.1382 & 46.846 & 46.438 & 36.136 & 42.0438 & 30.2139 & \textcolor{red}{49.6456} \\ \hline
% \multirow{6}{*}{VideoLQ} 
%  & BRISQUE $\downarrow$ & 29.605 & 26.4025 & 22.337 & 24.790 & 25.101 & 29.6062 & 42.581 & \textcolor{red}{23.0393} \\ 
%  & MUSIQ $\uparrow$ & 53.138 & 58.9585 & 52.975 & 59.4750 & 57.4886 & 53.0915 & 49.3046 & \textcolor{red}{63.8463}\\
%  & CLIPIQA $\uparrow$ & 0.334 & 0.499 & 0.478 & 0.3930 & 0.3772 & 0.3145 & 0.3328 & \textcolor{red}{0.567}\\
%  & MANIQA $\uparrow$ & -- & 0.2542 & -- & 0.3115 & 0.3275 & 0.2542 & 0.2682 & \textcolor{red}{0.3442}\\
%  & \(E_\text{warp}\) $\downarrow$ & 7.58 & 8.406 & 8.43 & 8.1075 & 7.586 & 7.409 & 7.28 & 7.897 \\
%  & DOVER $\uparrow$ & -- & 37.58 & 30.47 & 34.7721 & 36.86 & 31.8992 & 29.40 & \textcolor{red}{38.5054} \\ \hline
% \end{tabular}
% }
% % 70.734 (mgld); 42.0438
% % 72.0992 (progressive); 48.5205
% % 64.101 (ose_pure); 42.1382
% % 
% \vspace{10pt}
% \caption{Comparison of various methods across different datasets. This table is left blank for future data entry.}
% \label{tab:comparison}
% \end{table}



\noindent\textbf{Qualitative Comparison.}
To further demonstrate the effectiveness of DLoRAL, we visualize the Real-VSR results in Fig.~\ref{fig:comparison}. 
One can see that DLoRAL can remove complex spatial-variant degradations and generate realistic details,  significantly outperforming other Real-VSR models. 
Specifically, for the severely degraded facial region (first row), RealBasicVSR fails to reconstruct the facial structural, and Upscale-A-Video and STAR lose facial details. MGLD produces sharper outputs, but suffers from severe structural distortions, particularly around the eye regions. In contrast, DLoRAL successfully recovers fine facial features while maintaining structural integrity. 
The second row highlights the performance in texture reconstruction, where our method restores sharper and more legible texture patterns compared to the blurry or distorted outputs from other algorithms. 
% To demonstrate the effectiveness of DLoRAL, we visualize the VSR results on real-world VSR dataset in Fig~\ref{fig:comparison}. One can see that DLoRAL can remove complex spatial-variant degradations and generate realistic details, outperforming other state-of-the-art real-world VSR algorithms. Specifically, for the severe degradation in the first row, DLoRAL can well reconstruct the details while maintaining the structure of human face. As shown in the second row of~\ref{fig:comparison}, DLoRAL reconstructs
% clearer patterns than competing methods. More visual comparisons can be found in the \textbf{supplementary materials}.


To better compare the consistency, we plot the temporal profiles of the VSR results produced by competing methods Fig.~\ref{fig:temporal_consistency}. 
Real-ISR approaches such as StableSR and OSEDiff restore sharper details but suffer from severe temporal instability, as shown by the erratic fluctuations in their profiles, resulting in unpleasant flickering that harms the video quality.
On the other hand, while existing Real-VSR methods can offer better temporal consistency than Real-ISR methods, this comes at the cost of blurred details (see the results of Upscale-A-Video, MGLD and STAR in the left case of Fig.~\ref{fig:temporal_consistency}) or intra-frame artifacts (see the results of RealBasicVSR, Upscale-A-Video and STAR in the right case of Fig.~\ref{fig:temporal_consistency}).
In comparison, our DLoRAL produces smooth and stable transitions across frames, as reflected by its consistent temporal profiles. This qualitative evidence aligns with our quantitative results, demonstrating DLoRAL’s ability to preserve fine visual details while ensuring natural temporal consistency.
More visual comparisons can be found in the \textbf{Appendix}.


% Conversely, our DLoRAL algorithm achieves stable and coherent transitions across frames, as demonstrated in the smooth temporal evolution of reconstructed content. This qualitative assessment corroborates our quantitative measurements, confirming that our framework successfully achieves the dual objectives of preserving fine visual details while maintaining natural temporal coherence.


% Existing Real-VSR methods can ensure frame-to-frame consistency and stability but often at the cost of blurred edges or missing details. For instance, STAR, which achieves the best $E_{warp}$ across multiple datasets, suffers from noticeable blurring in edges and fine details. On the other hand, Real-ISR methods (\textit{e.g.,} StableSR and OSEDiff) are capable of restoring relatively sharper details but exhibit significant temporal instability, as evidenced by the erratic fluctuations in their temporal profiles. 
% To better compare the consistency of our method, we illustrate the temporal profiles of the VSR results produced by different algorithms in Fig.~\ref{fig:temporal_consistency}.
% Real-ISR methods such as StableSR and OSEDiff demonstrate significant temporal instability, evidenced by erratic fluctuations in their temporal profiles. These visual artifacts correspond to the flickering effects commonly observed in frame-by-frame processing. 
% Conversely, our DLoRAL algorithm, along with other temporal-aware methods, produces stable and coherent transitions across frames, as visible in the smooth temporal evolution of reconstructed content. This qualitative assessment corroborates our quantitative measurements, demonstrating that our framework successfully achieves the dual objectives of preserving fine visual details while maintaining natural temporal coherence.
% Additional visual comparisons covering various degradation types and content categories can be found in the \textbf{supplementary materials}.


\begin{figure}[!htb] % h: 当前位置, t: 顶部, b: 底部, p: 浮动页
    \centering
    \includegraphics[width=1.0\textwidth]{images/visual_comparison_onlyvideo_0514_1826_drawio.pdf} % 调整宽度为文档宽度的80%
   \vspace{-20pt}
    \caption{Qualitative comparison of VSR models on real-world VideoLQ dataset.} % 图片标题
    \label{fig:comparison} % 给图片加一个标签，用于引用
\vspace{-2pt}
\end{figure}


\begin{figure}[!htb] % h: 当前位置, t: 顶部, b: 底部, p: 浮动页
    \centering
    \includegraphics[width=1.0\textwidth]{images/consistency_comparison_v3_0516.pdf} % 调整宽度为文档宽度的80%
    \vspace{-15pt}
    \caption{Temporal profiles of competing Real-ISR and Real-VSR methods.} % 图片标题
    \label{fig:temporal_consistency} % 给图片加一个标签，用于引用
\vspace{2pt}
\end{figure}

\begin{table}[!htb]
\centering
\tiny
\setlength{\tabcolsep}{3pt} % 调整列间距
\renewcommand{\arraystretch}{1.2} % 调整行间距
\resizebox{0.9\textwidth}{!}{ % 自动缩放表格宽度
\begin{tabular}{|c||c|c||c|c|c|c|}
\hline
\multirow{2}{*}{} & \multicolumn{2}{c||}{Real-ISR Methods} & \multicolumn{4}{c|}{Real-VSR Methods} \\
\cline{2-7}
& StableSR  & OSEDiff 
& Upscale-A-Video & MGLD & STAR & \textbf{DLoRAL} \\ \hline
Inference Step & 200 &  1
& 30 & 50 & 15 & 1 \\ \hline
Inference Time (s/50 frames) & 32800 &  340
& 3640 & 4146 & 2830 & 346 \\ \hline
\# Total Param (M) & 1150 & 1294 
& 14442 & 1430 & 2492 & 1300 \\ \hline
\end{tabular}
}
\vspace{5pt}
\caption{Complexity comparison among different methods. All methods are evaluated using 50 $512 \times 512$ frames for the $\times$4 VSR task. Inference time is measured on an A100 GPU and includes the entire pipeline: data loading, processing, and result storage.}
\label{tab:complexity_comparison}
\vspace{-3mm}
\end{table}

\noindent\textbf{Complexity Comparison.}
We compare the inference steps, model size, and inference time of competing diffusion-based models in Tab.~\ref{tab:complexity_comparison}. The inference time of the whole pipeline (including data loading, data processing, and result storage) is reported, which is measured on the $\times$4 VSR task with 50 frames of $512 \times 512$ LQ images on a single NVIDIA A100 80G GPU. 
% Compared with Real-ISR methods, DLoRAL delivers a compelling quality-complexity balanced performance. Although its inference time (346s) is similar to OSEDiff (340s), DLoRAL achieves much better performance on visual quality and temporal consistency, as discussed in previous subsections.
Compared with Real-ISR methods, DLoRAL  (346s) achieves a strong balance between quality and complexity, delivering superior visual quality and temporal consistency while maintaining a similar speed to OSEDiff (340s).
Among the Real-VSR methods, DLoRAL achieves the fastest inference time and the lowest parameter count, benefiting from its efficient one-step design. Specifically, DLoRAL is more \textbf{10$\times$ faster} than Upscale-A-Video, MGLD, and \textbf{8$\times$ faster} than STAR, while maintaining superior visual quality.

% 

% We compare the inference step, the number of parameters, and inference time of competing diffusion-based SR
% models in Tab~\ref{tab:complexity_comparison}. The inference time is measured on the ×4 VSR task using 100 frames of 128 × 128 LQ images on a single NVIDIA A100 80G GPU. Among Real-VSR diffusion-based models, DLoRAL has the fewest parameters and fewest inference time beneficial from one-step characteristic. Specifically, DLoRAL is approximately 10 faster than Upscale-A-Video, MGLD and STAR. This further demonstrates our efficiency.


\noindent\textbf{User Study.}
We also conduct a user study to further examine the effectiveness of DLoRAL in comparison with existing RealVSR methods. We invited ten volunteers to participate in a user study. Our DLoRAL method was compared with the other three diffusion-based Real-VSR methods: Upscale-A-Video~\cite{zhou2024upscale}, MGLD~\cite{yang2024motion} and STAR~\cite{xie2025star}. We randomly selected 12 real-world LQ videos with complex degradations and motions from the VideoLQ dataset~\cite{chan2022realbasicvsr}, whose scenes are shown in Fig.~\ref{fig:illustration_user_study}(a). 
Each LQ video and its corresponding HQ videos generated by the competing Real-VSR methods were presented to the participants who were asked to select the best HQ result by considering two equally weighted factors: the perceptual quality and temporal consistency of the video.

The results of the user study are shown in Fig.~\ref{fig:illustration_user_study}(b). DLoRAL received \textbf{93} votes, significantly outperforming the other methods, with MGLD, STAR, and Upscale-A-Video receiving 14, 8, and 5 votes, respectively. This overwhelming preference for DLoRAL highlights its effectiveness in addressing the challenges of real-world video restoration. Note that the selected videos include a variety of motion scenarios. In scenarios with complex motion, DLoRAL is able to achieve superior visual quality while maintaining temporal consistency comparable to other methods. In relatively static scenes, DLoRAL demonstrates stable temporal consistency along with equally sharp and clear visual quality. 

\begin{figure}[htbp] % h: 当前位置, t: 顶部, b: 底部, p: 浮动页
    \centering
    \includegraphics[width=1.0\textwidth]{appendix_images/illustration_v2.pdf} % 调整宽度为文档宽度的80%
    \caption{LQ videos used in our user study and the voting results.} % 图片标题
    \label{fig:illustration_user_study} % 给图片加一个标签，用于引用
\vspace{-5pt}
\end{figure}
